EONSim: An NPU Simulator for On-Chip Memory and Embedding Vector Operations

Embedding vector operations are a key component of modern deep neural network workloads. Unlike matrix operations with deterministic access patterns, embedding vector operations exhibit input data-dependent and non-deterministic memory accesses. Existing neural processing unit (NPU) simulators focus on matrix computations with simple double-buffered on-chip memory systems, lacking the modeling capability for realistic embedding behavior. Next-generation NPUs, however, call for more flexible on-chip memory architectures that can support diverse access and management schemes required by embedding workloads. To enable flexible exploration and design of emerging NPU architectures, we present EONSim, an NPU simulator that holistically models both matrix and embedding vector operations. EONSim integrates a validated performance model for matrix computations with detailed memory simulation for embedding accesses, supporting various on-chip memory management policies. Validated against TPUv6e, EONSim achieves an average inference time error of 1.4\% and an average on-chip memory access count error of 2.2\%.

==> floats/float-eval-dlrm.tex <==
\begin{figure*}[t!]
    \centering
    \subfloat[Speedup]{
        \includegraphics[width=0.3\textwidth]{figures/dlrm-perf.pdf}
        \label{fig:eval_dlrm_perf}
    }
    \hfill
    \subfloat[On-chip memory access ratio]{
        \includegraphics[width=0.3\textwidth]{figures/dlrm-onmem.pdf}
        \label{fig:eval_dlrm_onmem}
    }
    \hfill
    \subfloat[Comparison of cache hit and miss counts between EONSim and ChampSim]{
        \includegraphics[width=0.3\textwidth]{figures/val-memaccess-champ.pdf}
        \label{fig:eval_val_memacc_champ}
    }
    \caption{Performance, on-chip memory access ratio, and cache behavior comparison for recommendation model inference workload.}
    \label{fig:eval_dlrm}
\end{figure*}


% \begin{figure}[t!]
%     \centering
%     \subfloat[Speedup]{\includegraphics[width=0.4\columnwidth]{figures/dlrm-perf.pdf}
%     \label{fig:eval_dlrm_perf}}
%     ~
%     \subfloat[On-chip memory access ratio]{\includegraphics[width=0.45\columnwidth]{figures/dlrm-onmem.pdf}
%     \label{fig:eval_dlrm_onmem}}    
%     ~
%     \caption{Performance and on-chip memory access ratio comparison for recommendation model inference workload.
%     }
%         \hfill
%     \subfloat[Comparison of cache hit and miss counts between EONSim and ChampSim]{
%         \includegraphics[width=0.35\textwidth]{figures/val-memaccess-champ.pdf}
%         \label{fig:eval_val_memacc_champ}
%     }
%     \label{fig:eval_dlrm}
% \end{figure}

==> floats/float-eval-validation-onmem.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/val-onmem.pdf}
    \caption{Number of cache hits for two cache replacement policies and three input traces using ChampSim (Champ) and EONSim (EON).
    }
    \label{fig:eval_val_onmem}
\end{figure}

==> floats/float-eval-vdb.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[Speedup]{\includegraphics[width=0.52\columnwidth]{figures/vdb-perf.pdf}
    \label{fig:eval_vdb_perf}}
    ~
    \subfloat[On-chip memory access ratio]{\includegraphics[width=0.48\columnwidth]{figures/vdb-onmem.pdf}
    \label{fig:eval_vdb_onmem}}    
    ~
    \caption{Performance and on-chip memory access ratio comparison for vector database search workload.
    }
    \label{fig:eval_vdb}
\end{figure}

==> floats/float-motiv-npuarch.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.70\columnwidth]{figures/npuarch.pdf}
    \caption{Baseline NPU architecture. An accelerator consists of an off-chip memory, a global buffer, and cores.
    % Each core contains dedicated units for scalar, vector, and matrix operations.
    }
    \label{fig:npu}
\end{figure}

==> floats/float-twofigs.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[This is figure A.]{\includegraphics[width=0.70\columnwidth]{figures/motiv_embops_bag.pdf}
    \label{fig:motiv_embops_bag}}

    \subfloat[This is figure B.]{\includegraphics[width=0.70\columnwidth]{figures/motiv_embops_ivf.pdf}
    \label{fig:motiv_embops_ivf}}
    
    \caption{These are figures.
    }
    \label{fig:motiv_embops}
\end{figure}

==> floats/tbl-eval-validation-onmem.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{1.2}
\caption{
Number of cache hits for two cache replacement policies and three input traces using ChampSim and EONSim
}
\label{table:eval_val_onmem}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
 &
  \textbf{\begin{tabular}[c]{@{}c@{}}ChampSim\\ LRU\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}EONSim\\ LRU\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}ChampSim\\ SRRIP\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}EONSim\\ SRRIP\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Reuse High}} & 1,266,627 & 1,266,627 & 1,320,706 & 1,320,706 \\ \hline
\multicolumn{1}{|c|}{\textbf{Reuse Mid}}  & 869,170   & 869,170   & 936,032   & 936,032   \\ \hline
\multicolumn{1}{|c|}{\textbf{Reuse Low}}  & 154,689   & 154,689   & 230,774   & 230,774   \\ \hline
\end{tabular}%
}
\end{table}
